SwissADT: An Audio Description Translation System for Swiss Languages

Audio description (AD) is a crucial accessibility service provided to blind persons and persons with visual impairment, designed to convey visual information in acoustic form. Despite recent advancements in multilingual machine translation research, the lack of well-crafted and time-synchronized AD data impedes the development of audio description translation (ADT) systems that address the needs of multilingual countries such as Switzerland. Furthermore, since the majority of ADT systems rely solely on text, uncertainty exists as to whether incorporating visual information from the corresponding video clips can enhance the quality of ADT outputs. In this work, we present SwissADT, the first ADT system implemented for three main Swiss languages and English. By collecting well-crafted AD data augmented with video clips in German, French, Italian, and English, and leveraging the power of Large Language Models (LLMs), we aim to enhance information accessibility for diverse language populations in Switzerland by automatically translating AD scripts to the desired Swiss language. Our extensive experimental ADT results, composed of both automatic and human evaluations of ADT quality, demonstrate the promising capability of SwissADT for the ADT task. We believe that combining human expertise with the generation power of LLMs can further enhance the performance of ADT systems, ultimately benefiting a larger multilingual target population.

==> latex/tables/chde-article.tex <==
\begin{table}[!htb]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{ll}
        \toprule
         Language & Example \\
         \midrule
         CH-DE & \textbf{De} Schorsch und \textbf{d} Claudia sind beidi Mitti 30i.  \\
         DE & \sout{Der} Schorsch und \sout{die} Claudia sind beide Mitte 30. \\
         EN & Schorsch and Claudia are both in their 30s. \\
         \bottomrule
    \end{tabular}
    }
    \caption{Presence of articles in different languages.}
    \label{tab:chde-article}
\end{table}
